GRAthena++: puncture evolutions on vertex-centered oct-tree AMR

Numerical relativity is central to the investigation of astrophysical sources in the dynamical and strong-field gravity regime, such as binary black hole and neutron star coalescences. Current challenges set by gravitational-wave and multi-messenger astronomy call for highly performant and scalable codes on modern massively-parallel architectures. We present GR-Athena++, a general-relativistic, high-order, vertex-centered solver that extends the oct-tree, adaptive mesh refinement capabilities of the astrophysical (radiation) magnetohydrodynamics code Athena++. To simulate dynamical space-times GR-Athena++ uses the Z4c evolution scheme of numerical relativity coupled to the moving puncture gauge. We demonstrate stable and accurate binary black hole merger evolutions via extensive convergence testing, cross-code validation, and verification against state-of-the-art effective-one-body waveforms. GR-Athena++ leverages the task-based parallelism paradigm of Athena++ to achieve excellent scalability. We measure strong scaling efficiencies above $95\%$ for up to $\sim 1.2\times10^4$ CPUs and excellent weak scaling is shown up to $\sim 10^5$ CPUs in a production binary black hole setup with adaptive mesh refinement. GR-Athena++ thus allows for the robust simulation of compact binary coalescences and offers a viable path towards numerical relativity at exascale.

==> Makefile <==
# make sure to use bash on Debian/Ubuntu, not dash
SHELL := /bin/bash

SRC = paper20210120
FIGURES =

# temporarily add generated bib
GENBIB := $(shell cat references.bib \
                  references_supplementary.bib > references_generated.bib)

all: \
 $(SRC).pdf
paper: $(SRC).pdf

%.pdf: %.tex
	pdflatex $*
	bibtex $* ; \
	pdflatex -nonstopmode $* ; \
	pdflatex -nonstopmode $*

clean:
	rm -f $(SRC).{pdf,aux,bbl,blg,dvi,log,out,toc,synctex.gz}
	rm -f *~
	# add temporarily
	rm -f references_generated.bib
	rm -f paperNotes.bib

new: clean all

.PHONY: all clean new

